Modeling and Simulation of a Fluttering Cantilever in Channel Flow

Characterizing the dynamics of a cantilever in channel flow is relevant to applications ranging from snoring to energy harvesting. Aeroelastic flutter induces large oscillating amplitudes and sharp changes with frequency that impact the operation of these systems. The fluid-structure mechanisms that drive flutter can vary as the system parameters change, with the stability boundary becoming especially sensitive to the channel height and Reynolds number, especially when either or both are small. In this paper, we develop a coupled fluid-structure model for viscous, two-dimensional channel flow of arbitrary shape. Its flutter boundary is then compared to results of two-dimensional direct numerical simulations to explore the model's validity. Provided the non-dimensional channel height remains small, the analysis shows that the model is not only able to replicate DNS results within the parametric limits that ensure the underlying assumptions are met, but also over a wider range of Reynolds numbers and fluid-structure mass ratios. Model predictions also converge toward an inviscid model for the same geometry as Reynolds number increases.

==> sections/sec4.tex <==
% %\subsection{Dynamic Mode Decomposition} %\label{sec:DMD} 
% In order to evaluate the linear stability of the FSI system, We employ an empirical approach based on the Dynamic Mode Decomposition (DMD) to calculate growth/decay rates, frequencies, and mode shapes directly from the (nonlinear) simulation data \citep{needrefs}. DMD is a data decomposition technique that approximates the eigenmodes of the linear operator that best describes the dynamics of the system, i.e. from one time instance to the next \citep{Schmid2010,Chen2012}.  

% \tim{Taira and others have discussed applying DMD for stability analysis..I think it would be more appropriate to reference those rather than Towne}

%Developed over the last decade \citep{Schmid2010} as an alternative or complement to POD, it provides a means of assessing the time coherent, large scale structures as a linear map that does not require modes to be orthogonal.  
% The linear map is also fully described by a single eigenvalue per degree-of-freedom, which encompasses one growth- or decay- rate and one frequency per mode. 
%This highlights that time, not space, is orthogonalized in the method \citep{Towne2018,Schmid2010}.  Another notable result by \citeauthor{Chen2012} \citep{Chen2012} establishes the equality of DMD to the discrete Fourier transform (DFT) in zero-mean periodic data, when snapshots are linearly consistent \footnote{This is when snapshots, or the columns of the data matrix, share the same nullspace.}. 
% We employ DMD to calculate growth/decay rates and frequencies of the beam in the FSI DNS simulations, which are compared to the quasi-1D model eigenvalues.  DMD modes are analogous to quasi-1D eigenmodes, and their shapes qualitatively compared.      
% \begin{figure}[h!]
%     \centering
%    \includegraphics[trim={.5cm 6cm .5cm 6cm},clip,width=1\textwidth]{figures/BeamDiscData.pdf}
%         \caption{Illustration of elastic member displacement and discrete formulation of data matrix elements.}  
%      \label{fig:DataMatrixBeamFig}
% \end{figure} 
We choose the transverse displacement $\delta$, illustrated in figure \ref{fig:NozzleDiffuserGeometryl}, as the primary quantity to characterize the fluid-structure system dynamics.  

\tim{Unless you invented something in the analysis that follows, it goes in an appendix and you simply state here in words the algorithms you applied, giving some flavor about the rank issues you discuss}

% The Lagrangian coordinate $s$ follows the arc length of the beam, with $\mathrm{\hat{y}}$ displacement at discrete $s_i$ ($i \in \mathbb{Z}: [1,p]$) and time $t_j$  ($j \in \mathbb{Z}: [1,n]$ ) as $\delta(s_i,t_j) = \delta^{(j)}_i$.  We define the data matrix $\mathbf{X}$, 

% \begin{equation} \label{eq:DataMatrix}
% \mathbf{X} = \begin{bmatrix}
%  	\delta_1^{(1)} & \delta_1^{(j)} & \dots  & \delta_1^{(n)} \\
%     \delta_i^{(1)} & \delta_i^{(j)} & \dots  & \delta_i^{(n)} \\
%     \vdots & \vdots & \ddots & \vdots \\
%     \delta_p^{(1)} & \delta_p^{(j)} & \dots  & \delta_p^{(n)}
% \end{bmatrix} \in \mathbb{R}^{p\times n}.
% \end{equation}  

% The rows of $\mathbf{X}$ are measurements of points along the beam, and the columns are the time series for each point with size $\Delta t$. For typical fluid applications, $p \gg n$, as the discretization of the fluid-domain requires a large number of points as compared to the number of time steps analyzed. However,  $p \ll n$ for our system as $i$ only spans the one-dimensional beam discretization.  Specifically, $p \sim 10^2$ while $n \sim \left[10^4 - 10^5 \right]$ for our $\mathbf{X}$ matrices processed.  This poses issues due to rank limitations of $\mathbf{X}$ when calculating DMD eigenvalues, as they become very susceptible to variations in the time segment length (as seen in \cite[pg.~12]{Tu2013}).  To overcome this, we implement an augmented data matrix as typically done in the eigensystem realization algorithm (ERA).  ERA was developed in the controls community to identify the lowest order linear operator that describes an output data set from specified inputs.  \citeauthor{Tu2013} in \cite[pg.~20--23]{Tu2013} describe the connection between DMD and ERA modes, and the benefits of augmenting the data matrix as in input matrix $\mathbf{H}$ and output matrix $\mathbf{H}'$,

% \begin{equation} \label{eq:DMDInOutMatrix}
% \mathbf{H}' = \begin{bmatrix}
%  	 {\delta}_1^{(1)} &  {\delta}_1^{(l)} & \dots  &  {\delta}_1^{(N)} \\
%      {\delta}_k^{(1)}  &  {\delta}_k^{(l)} & \dots  &  {\delta}_k^{(N)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_p^{(1)} &  {\delta}_p^{(l)} & \dots  &  {\delta}_p^{(N)} \\
%      {\delta}_{p+1}^{(1)} &  {\delta}_{p+1}^{(l)} & \dots  &  {\delta}_{p+1}^{(N)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{2p}^{(1)} &  {\delta}_{2p}^{(l)} & \dots  &  {\delta}_{2p}^{(N)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{\left( \frac{n}{N} \right) p}^{(1)} &  {\delta}_{\left( \frac{n}{N} \right)p}^{(l)} & \dots  &  {\delta}_{\left( \frac{n}{N} \right)p}^{(N)} \\
% \end{bmatrix} \in \mathbb{R}^{\left( \frac{n}{N} \right)p \times N} , \
% \mathbf{H} = \begin{bmatrix}
%  	 {\delta}_1^{(2)} &  {\delta}_1^{(l+1)} & \dots  &  {\delta}_1^{(N+1)} \\
%      {\delta}_k^{(2)}  &  {\delta}_k^{(l+1)} & \dots  &  {\delta}_k^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_p^{(2)} &  {\delta}_p^{(l+1)} & \dots  &  {\delta}_p^{(N+1)} \\
%      {\delta}_{p+1}^{(2)} &  {\delta}_{p+1}^{(l)} & \dots  &  {\delta}_{p+1}^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{2p}^{(2)} &  {\delta}_{2p}^{(l+1)} & \dots  &  {\delta}_{2p}^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{\left( \frac{n}{N} \right) p}^{(2)} &  {\delta}_{\left( \frac{n}{N+1} \right)p}^{(l+1)} & \dots  &  {\delta}_{\left( \frac{n}{N} \right)p}^{(N+1)} \\
% \end{bmatrix} \in \mathbb{R}^{\left( \frac{n}{N} \right)p \times N} ,
% \end{equation}
% where $l \in \mathbb{Z}: [1,N]$, $ p < N \le n \in \mathbb{Z}$ is the total number of snapshots in each time series block, $k \in \mathbb{Z}: [1,\left( \frac{n}{N} \right)p]$ is the index for the  augmented states.  Matrix $\mathbf{H}$ is the input matrix, and  a segmented version of the time series of $\mathbf{X}$: we have defined a new time series length $N < n$, divided the original into blocks and appended each block to the columns of $\mathbf{H}$.  We choose $N > \frac{n}{N}p$ such that $k$ is still the small dimension, with typical values of $\frac{n}{N}$ used range from 1 to 4 at most.  
% \begin{equation} \label{eq:DMDOutputMatrix}
% \mathbf{H} = \begin{bmatrix}
%  	 {\delta}_1^{(2)} &  {\delta}_1^{(l+1)} & \dots  &  {\delta}_1^{(N+1)} \\
%      {\delta}_k^{(2)}  &  {\delta}_k^{(l+1)} & \dots  &  {\delta}_k^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_p^{(2)} &  {\delta}_p^{(l+1)} & \dots  &  {\delta}_p^{(N+1)} \\
%      {\delta}_{p+1}^{(2)} &  {\delta}_{p+1}^{(l)} & \dots  &  {\delta}_{p+1}^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{2p}^{(2)} &  {\delta}_{2p}^{(l+1)} & \dots  &  {\delta}_{2p}^{(N+1)} \\
%     \vdots  & \vdots & \ddots & \vdots \\
%      {\delta}_{\left( \frac{n}{N} \right) p}^{(2)} &  {\delta}_{\left( \frac{n}{N+1} \right)p}^{(l+1)} & \dots  &  {\delta}_{\left( \frac{n}{N} \right)p}^{(N+1)} \\
% \end{bmatrix} \in \mathbb{R}^{\left( \frac{n}{N} \right)p \times N} ,
% \end{equation}
?
% Hence, we must understand from the data set which DMD eigenvalue eigenmode pair best represents it.  Assuming the underlying dynamics come from a linear time-invariant system, the physically meaningful eigenvalues should remain fixed in time. Therefore, by varying the time segment for which we define $\mathbf{X}$ (along with $\mathbf{H}$ and $\mathbf{H'}$), we can discern physical modes as those that are associated with invariant eigenvalues.  Let $\mathbf{X}_1$ and $\mathbf{X}_2$ be different data matrices as defined in equation \ref{eq:DataMatrix}, both as subsets of a single time series for the beam.  
% Let $\lambda_l$ be the DMD spectrum of $\mathbf{X}_1$ and $\lambda_q$ that of $\mathbf{X}_2$.  A mode $\mathbf{\hat{u}}_l$ is physically meaningful if its corresponding $\lambda_l$  meets the condition
% \begin{equation} \label{eq:physsigcriteria}
% \min_q \left[|\lambda_l - \lambda_q|\right] < D,
% \end{equation}
% where $D$ is the invariant tolerance and defined as 1E-2 for our cases.  Once physically meaningful eigenvalues have been determined, we track the least stable eigenvalue $\lambda_{\mathrm{max}} = \max_{\lambda_m} \left\{ \text{Re}\left[ \lambda_m \right] \right\}$, where $\lambda_m$ is the set of $\lambda_l$ that meets criteria  \ref{eq:physsigcriteria} ($m \le l$).  
% The last step is to check whether $\lambda_{\mathrm{max}}$ captures what is observed as the dynamics of the tip response, $\delta_p^{(j)}$. This is done by fitting a exponential to the peaks of $\delta_p^{(j)}$, and taking a DFT of the demodulated signal, such that the segment is represented by 
% \begin{equation}
% \delta^{(j)}_p \sim \mathrm{e}^{\zeta j \Delta t } \cos\left( \omega_{\mathrm{max}} j \Delta t \right).
% \end{equation}
% The signal phase and absolute amplitude are not necessarily relevant for our comparison, only the amplitude growth/decay $\zeta$ and the oscillating frequency $\omega_{\mathrm{max}}$.  We compare $\zeta$ to Re$\left[ \lambda_{\mathrm{max}} \right]$ and $\omega_{\mathrm{max}}$ to Im$\left[ \lambda_{\mathrm{max}} \right]$.  If the system is dominated by a single frequency response, this gives us confidence that we have obtained the correct DMD eigenvalue and eigenmode pair.  If more than one more dominates the response, the check provides a general search area for the decay rate and dominant frequencies.  If no $\lambda_l$ meets criteria \ref{eq:physsigcriteria}, we increase the $\frac{n}{N}$ ratio and iterate.  Similarly, we may iterate with a longer time series that captures the linear portion of the dynamics better, for example.  

% Figures \ref{fig:DataSetFull}, \ref{fig:DataSetExpDFTFit}, and  \ref{fig:DMDEigValswithFit} illustrate this procedure for an example data set from a stable, constant channel flow FSI DNS simulation discussed in detail in section \ref{sec:ConstChannelFlow}.  Figure \ref{fig:DataSetFull} shows the full time series of two beam locations, the tip at $\delta_p$ and at the beam half-way point, $\delta_{p/2}$. Two subsets of the full time series are also shown for the two beam location, where $T_1 > T_2$ are time shifts to obtain each subsegment. The data matrices $\mathbf{X}_1$ for segment with a time shift $T_1$ and $\mathbf{X}_2$ for a time shift $T_2$, are built from equation \ref{eq:DataMatrix}, and their respective $\mathbf{H'}$ and $\mathbf{H}$ follow from equations \ref{eq:DMDInOutMatrix} and \ref{eq:DMDInOutMatrix}.  The exponential fit and power spectral density for the tip displacement in the $\mathbf{X}_1$ are shown in figure \ref{fig:DataSetExpDFTFit}, with $\zeta = -0.011$ and $\omega_{\mathrm{max}} = 3.77$.  Figure \ref{fig:DMDEigValswithFit} then compares the positive frequency DMD eigenvalues and the fit parameters $\zeta$ and $\omega_{\mathrm{max}}$.              

% \begin{figure}[tbh!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%    	\includegraphics[width=1\textwidth]{figures/Sim6_FullT_0Data.pdf}
%         \caption{} \label{fig:aseg} 
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%    	\includegraphics[width=1\textwidth]{figures/Sim6_FullT_1Data.pdf}
%         \caption{ }  \label{fig:bseg}
%     \end{subfigure}
%     \caption{Stable beam time series at the beam tip, $\delta_p$ and at beam midpoint, $\delta_{p/2}$. The figure illustrates a segment data set $\mathrm{X}_1$ (\ref{fig:aseg}) and $\mathrm{X}_2$ (\ref{fig:bseg}) with a time shift of $T_1 > T_2$, respectively.} \label{fig:DataSetFull}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%    	\includegraphics[width=1\textwidth]{figures/Sim6_Tseg_0Data.pdf}
%         \caption{} \label{fig:aseg1} 
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%    	\includegraphics[trim={0cm 0cm 2cm .25cm},clip,width=1\textwidth]{figures/Sim6_DFT_Data0.pdf}
%         \caption{ }  \label{fig:bseg1}
%     \end{subfigure}
%     \caption{Beam tip $\delta_p^{(j)}$ for $\mathbf{X}_1$ segment. The figure illustrates the exponential fit (\ref{fig:aseg1}) with a $\zeta = -0.0111$ and the DFT  of the demodulated signal (\ref{fig:bseg1}) with $\omega_{\mathrm{max}} = 3.77$. } \label{fig:DataSetExpDFTFit}
% \end{figure}
         
         
% \begin{figure}[H]
%     \centering
%    \includegraphics[width=1\textwidth]{figures/DMDSpectrum_Combo_0Data.pdf}
%         \caption{Comparison of DMD eigenvalues (shown for Im$\left[ \lambda\right] > 0$ ) and fit pair $(\zeta, \omega_{\mathrm{max}})$ from the beam tip time series. }  
%      \label{fig:DMDEigValswithFit}
% \end{figure} 

% In practice, if the system is dominated by a single eigenmode eigenvalue pair, as in the example, proceeding with the algorithm in reverse order may be desirable: by finding $\zeta$ and $\omega_{\mathrm{max}}$ that describe the tip displacement first, $\lambda_{\mathrm{max}}$ can be informed and narrowed, and the verification step becomes the comparison between $\mathrm{X}_1$ and $\mathrm{X}_2$ DMD spectra.

% Lastly, because of the $\mathbf{X}$ augmentation to produce $\mathbf{H}$ and $\mathbf{H}'$, $\hat{\mathbf{u}}_k \in \mathbb{C}^{ \frac{n}{N} p \times 1 } $.  In order to compare mode shapes with the quasi-1D model, we employ a similar procedure to ERA and restrict the observables to the first $p$ elements of $\hat{\mathbf{u}}_k$.  This is equivalent to producing a reduced order model from $\mathbf{H}$ with the same dimension as the output of the dynamical system represented by $\mathbf{X}$ \citep{Tu2013}. $\lambda_{m}$ and the restricted $\hat{\mathbf{u}}_{m}$ provide direct quantitative measures for a comparison between FSI DNS time series and the eigendecomposition of the quasi-1D model equations. 
